Push-MOG: Efficient Pushing to Consolidate Polygonal Objects for Multi-Object Grasping

Recently, robots have seen rapidly increasing use in homes and warehouses to declutter by collecting objects from a planar surface and placing them into a container. While current techniques grasp objects individually, Multi-Object Grasping (MOG) can improve efficiency by increasing the average number of objects grasped per trip (OpT). However, grasping multiple objects requires the objects to be aligned and in close proximity. In this work, we propose Push-MOG, an algorithm that computes "fork pushing" actions using a parallel-jaw gripper to create graspable object clusters. In physical decluttering experiments, we find that Push-MOG enables multi-object grasps, increasing the average OpT by 34%. Code and videos will be available at https://sites.google.com/berkeley.edu/push-mog.

==> figures/wksp_grouped.tex <==
\begin{figure}[t]
    \vspace{0.2cm}
    \centering
    {\includegraphics[width=85.5mm]{images/wksp_gropuped.jpg}}
    \caption{\textbf{A clustered workspace with the blocks clustered after a push action. The starting workspace was randomized, as seen in Fig.~\ref{fig:wksp_scatter}}}
\label{fig:wksp_grouped}
\end{figure}

==> figures/wksp_scattered.tex <==
\begin{figure*}
    \centering
    {\includegraphics[width=85mm]{images/groups.png}}
    \caption{\text{This figure shows the clustering formed by Push-MOG of an initial scene. The numbers on each cluster identify the order that the algorithm will perform the pushing and grasping actions.}}
\label{fig:wksp_scatter}
\end{figure*}


==> old_versions/results_general.tex <==
\begin{center}
\begin{table}[t]
\caption{Physical decluttering experimental results for random scenes, comparing baselines \textbf{Frictional SOG, MOG-Net}, and the method \textbf{\algo}. Experiments were conducted with a Robotiq 2F-85 parallel-jaw gripper mounted on a UR5 robot arm, on 5 random scenes of 34 objects, with the goal placed directly adjacent (see Figs \ref{fig:fig1} and  \ref{fig:wksp_scatter}).} %\textcolor{blue}{Rough computation: 1000 items, then Frictional SOG gets them all in $3$ hours, and Push-MOG gets them all in $4$ hours (if transports don't take extra time); FSOG takes $1000$ transports, P-MOG takes $750$. Thus for PMOG to be more efficient (in PPH) than FSOG, $250$ transports must take $\geq 1$ hour to perform, so transports must take $\geq 3600/250 = 14.4$ seconds. } } 
\centering 
% \begin{tabular}{@{}l@{\quad}c@{\quad}c@{\quad}c@{\quad} c@{}} 
\begin{tabular}{@{}l@{\quad} c@{\quad} c@{}}
% {|c|c|c|c|c|c|c|}
\toprule 
Methods & Transports per object (TPO) & Picks per hour (PPH)\\
% \midrule
Frictional SOG & 1.01 $\pm$ 0.014  & 331.70 $\pm$ 4.33\\
MOG-Net & 1.02 $\pm$ 0.039 & 325.23 $\pm$ 6.81\\
\algo & 0.75 $\pm$   0.087& 250.16 $\pm$  17.06 \\
% \algo~ \\
\bottomrule

%\multicolumn{2}{p{.35\textwidth}}{\vspace{0.1pc} \textcolor{blue}{Rough computation: 1000 items, then Frictional SOG gets them all in $\sim 3$ hours, and Push-MOG gets them all in $\sim 4$ hours}}

\end{tabular}
\label{tab:results}
\end{table}
\end{center}

% Frictional SOG & 331.70 $\pm$ 4.33 \\
% MOG-Net & 325.23 $\pm$ 6.81 \\
% Push-MOG & 250.16 $\pm$  17.06 \\

==> old_versions/section-1-introduction.tex <==
\section{Introduction}

%Many applications require fast and efficient robotic manipulation \cite{Fisac-ARXIV-2018, VILLANI-Mech-2018, Gomez-Access-2017}. Multi-Object Grasping (MOG) \cite{mogplane, mognet} can be more efficient than single-grasp algorithms. However, existing work in MOG assumes objects are clustered together, which does not hold in unstructured environments. 

Efficient object manipulation is {a key task in industrial, commercial, and domestic robotics, incorporating elements from foundational problems such as motion planning, grasping, and task planning
%
% It has been the primary topic of many prior works
%
\cite{GOMP, DJ-GOMP, Herbert-CDC-2017, Ichnowski-ICRA-2022}. 
%
\textcolor{blue}{In particular, many applications center on the task of transferring a collection of objects from a surface into a bin or basket (in this work we refer to it as the \emph{goal}), either for the purpose of clearing or decluttering the surface or preparing the objects for transportation to another location.} 
%
\textcolor{blue}{Efficiency at this task is typically measured in \emph{picks per hour} (PPH), which measures the rate at which objects are removed from the work space.}
%
\textcolor{blue}{Much prior work has focused on improving PPH by speeding up the robot's motions, without fundamentally altering the basic strategy of moving the objects one at a time; however, the alternative approach of removing multiple objects at once with \emph{multi-object grasping} (MOG) has received relatively little attention. MOG can provide better efficiency than traditional single-object grasping (SOG) \cite{mogplane, mognet}, especially when the goal is relatively far away.}
%
%Much of the research in the field has focused on \emph{faster} motion, which is generally measured using picks per hour (PPH).
%
%However, there has been little focus on increasing the transports-per-object (TPO), the average number of trips needed to clear an object (lower is better). TPO has the advantage of providing speedups in long-distance transport tasks. Grasping multiple objects simultaneously is another way to reduce transport actions. 
%
\textcolor{blue}{Prior work on MOG mainly focused on developing techniques (such as MOG-Net \cite{mognet}) for detecting and executing effective multi-object grasps in a scene. However, grasping multiple objects at once requires them to be close enough to all fit within the gripper width, which may be rare when the objects are arranged in an unstructured way (for instance, distributed randomly).}
%
%Prior work on multi-object grasping \cite{mognet} focused on objects that were not uniformly distributed on a table. When objects are uniformly distributed, it is difficult to directly find multi-object grasps given the width of parallel-jaw grippers. 
Thus, to create graspable object clusters, additional rearrangement actions like pushing \cite{Arruda-Humanoids-2017, Hogan2020} may be required.  

In this work, we propose \emph{\algo}, a picking system that uses pushes to increase the average number of objects that grasped at once. %when objects are uniformly distributed. 
%
\algo~uses hierarchical clustering to identify clusters of objects which could potentially be grasped together.
%
%specifically, the objects must have diameters whose sum is less than the gripper width, and they should be in relative physical proximity to each other. 
%
%\algo~then uses the gripper to push the objects in each cluster closer to each other to prepare them for grasping. 
%
Finally, MOG-Net is employed to find and execute good multi-object grasps in the rearranged scene. \textcolor{blue}{To execute stable pushes on polygonal objects with a parallel-jaw gripper, \algo~utilizes \emph{fork pushing}, in which the jaw is opened to an appropriate width and the object is pushed perpendicular to the jaw, thus enabling a variety of stable pushes (see Fig.~\ref{fig:polypush}).}
%

\textcolor{blue}{We also propose \emph{transports per object} (TPO) as a metric for evaluating the effectiveness of multi-object grasps. We define a \emph{transport} as an action where the robot moves the gripper to the goal and back to the workspace;\footnote{Generally it is carrying objects, but even if it misses a grasp and ends up carrying nothing it is still considered a transport.} thus, in SOG, the TPO is $1$ (or slightly more than $1$ due to failed grasp attempts), whereas the goal of MOG is to improve efficiency by reducing TPO. TPO can also be used to estimate how MOG affects the efficiency of decluttering (measured in PPH) for various goal distances -- in general, the further away the goal, the more valuable it is to reduce TPO.}
%
%We use hierarchical clustering to create clusters of objects. We make sure to have valid clusters before grasping. This is accomplished by making sure that the sum of the widths of all the polygonal objects inside the cluster is less than or equal to the width of the gripper. Once all our clusters are valid we randomly chose a cluster and plan pushing actions to efficiently rearrange objects within it. We repeat this process recursively until all of our clusters are rearranged. 

\textcolor{blue}{We test \algo~in a physical environment consisting of randomly-distributed polygonal objects on a flat surface, in which the robot executes both grasps and pushes using a parallel-jaw gripper, against two baselines: (i) Frictional SOG, which removes the objects in a random order one at a time; (ii) MOG-Net, which searches for multi-object grasps but does not apply rearrangement. We find that MOG-Net without rearrangement achieves a TPO of $\approx 1$, suggesting that naturally occurring good multi-object grasps are rare, while Push-MOG achieves a TPO of $0.75$, though at a cost of extra time for executing pushes. Since saving TPO is more valuable when the goal is farther away, \algo~can improve picking efficiency when transports are comparatively slow or expensive.}

%In physical experiments, we find that \algo~ efficiently generates multi-object grasps after pushing, and it compares fairly with multi-object grasping without pushing. We make the following contributions: 

%\begin{itemize}
%    \item [1.] \algo~ is an efficient algorithm that pushes objects to rearrange them within clusters and picks multiple objects at once. 
%    \item [2.] A push planning algorithm that exploits object geometry to generate stable pushes. 
%    \item [3.] Physical experiments comparing \algo~to baselines. 
%\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{images/fig1.jpg}
    \caption{ The decluttering problem is where objects must be transported to a packing box. We use pushes to efficiently rearrange uniformly distributed objects before picking them up with multi-object grasps.}
    \label{fig:fig1}
    \vspace{-5mm}
\end{figure}

==> old_versions/section-2-related-work.tex <==
\section{Related Work}
%In this section we review prior work on multi-object grasping, pushing, and point clustering. 

\subsection{Multi-object grasps} 

Early work on multi-object grasping \cite{Harada-ICRA-1998, Harada-TRA-2000, Yamada-ICRA-2005, Yamada-JCSE-2015} used multi-fingered robot hands and proposed conditions for a stable grasp of objects, 
%
%While these were the pioneering works on multi-object grasping, 
%
focusing on numerical simulations without physical robot multi-object grasps or a focus on automation. %In this work, we use a readily-available parallel-jaw gripper and propose a novel pushing action to allow more objects to be grasped simultaneously. %to increase PPH on a physical robot system.  
%
Chen et al. \cite{Chen-IROS-2021} propose a method for a robot to dip its gripper inside a pile of identical spherical objects, close it, and estimate the number of grasped objects. Shenoy et al.~\cite{Shenoy-CoRR-2021} focus on the same problem but with the goal of transferring the picked spherical objects to another bin. Our work is focused on efficiently rearranging scenes with pushes~\cite{Dogar-RSS-2011, Danielczuk-CASE-2018, Huang-IROS-2021, Agboh-Humanoids-2018} before multi-object grasping. Sakamoto et al. \cite{Sakamoto-IROS-2021} proposed such a picking system where the robot first uses pushing~\cite{largescalerearrange, Bejjani-IROS-2021, Mohammed-ICRA-2020}, to move one cuboid to the other and thereafter grasp both cuboids. Our approach handles any multi-sided object and focuses on large-scale problems where clustering is required to decide which objects to push and where. 

% \subsection{Planar Object Detection}\label{sec:cv}

%  Li et al. \cite{lowpoly} present a method to approximate general shapes using simple objects by using kinetic partitioning as the basis for merging and splitting the partitions. In this way simple and complex shapes can be captured. Due to the defined, objectal nature of our problem, we detect corners, contours, and harsh edges from a 2-Dimensional frame using OpenCV. We then convert them to robot coordinates through a transform using an ArUco marker \cite{aruco} on the workspace.


\subsection{Pushing} 
Robotic pushing has been used in prior work to move a target object to a goal location \cite{Hogan2020, Agboh-ISRR-2019}, rearrange a working surface \cite{king2016, Song-IROS-2020}, and retrieve items from cluttered shelves \cite{Huang-IROS-2021, Agboh-Humanoids-2018, Muhayyudin-RAL-2018}. %We take a similar approach and apply robotic pushing to the multi-object grasping problem, to rearrange scenes before picking to permit more objects to be grasped together. %thereby improving picks per hour. 

During robotic pushing, uncertainty in the state, control, and model can result in failures~\cite{Agboh-WAFR-2018, Agboh-arxiv-2021}. Prior work \cite{Yuan-ICRA-2018, Arruda-Humanoids-2017} has trained networks to generate robust pushing actions. Others have taken an open-loop approach to generate these robust pushes \cite{Goldberg-Algorithmica-1993, Erdmann1988}. For example, Johnson et. al. \cite{Johnson-RAL-2016} propose robustness metrics and use them to generate robust open-loop pushes. They exploit gripper and object geometries to generate these robust pushes. We take a similar open-loop pushing approach and leverage object and gripper geometries to generate robust pushes. 

% Pushing has been a topic of constant research in the field, where \cite{Sudsang-TASE-2002, Balorda-ICRA-199, Lloyd-TASE-2022, Deng-IROS-2019} explore methods to robustly push objects. \todo~add more

\subsection{Point Clustering}\label{sec:usup_clust}
Prior work in point clustering is well-established \cite{James2013, mirkin2005clustering}, specifically in the hierarchical variant \cite{heir, heirfast}, which aims to cluster data in an unsupervised fashion. This method constructs a distance-based tree that forms clusters of points from the bottom up which is then split at a `height' to determine the final clusters. 
%
Additional work by Dao et al. \cite{dao_constrain} explores clustering with human-defined constraints. It introduces the idea of simplifying and solving NP-Hard problems by constraining them through a limit on inter-cluster distance metrics, such as maximum cluster diameter, or within-cluster variation \cite{dao_constrain}. In this work, we use a distance-based hierarchical clustering algorithm but split object clusters to satisfy gripper width constraints. 

% This is done through a matrix representation of inter-point constraints, in which each set of agreeing points is ``represented'' by one point. This is then optimized over the human-defined constraints.

% \subsection{Push Action Planning}\label{sec:push_plan}
% \begin{itemize}
%     \item general push planning between two points
%     \item avoiding collisions with the object being pushed to
%     \item since many objects are being pushed to the same location, how do we handle collisions
% \end{itemize}

==> old_versions/section-3-problem-statement.tex <==
\section{Problem Statement} \label{sec:problem-statement}

In \cite{mogplane}, Agboh et al. studied the problem of using an overhead camera and a parallel-jaw gripper to transport a collection $O$ of extruded polygonal convex objects (prisms) from a flat work surface to a \emph{goal} (a bin or box located a little outside the workspace) by taking advantage of \emph{multi-object grasping}, in which multiple objects are grasped simultaneously and transported together to the goal area. 

% The objects are all assumed to be in a pose with two antipodal (possibly non-rectangular) sides parallel to the work surface and all other (rectangular) sides parallel to the work surface, allowing for the grasp and push actions to be considered as 2D problems (except when the manipulator tips over an object).

In this work, we extend this problem by adding the \emph{push} action, in which the gripper pushes an object\footnote{In this work we only consider pushing single objects. However, in the future, it may be interesting to consider using multi-object pushing and multi-object grasping together.} within the workspace; by doing so, the robot can arrange the objects to create more efficient grasps. Since pushing is faster to execute than grasping and the objects are typically closer to each other than to the goal, using pushes to facilitate multi-object grasps\footnote{Since the goal is a bin or box with raised walls, it is not possible to push the objects into it; they must be grasped, lifted, and carried there.} can reduce the number of transport actions needed to clear the objects. As in \cite{mognet} (Agboh et al.), we consider a frictional model of planar grasping, which not only corresponds better to real grasping problems but also permits a larger set of stable grasps, thus allowing the algorithm to access a wider range of potential solutions. 

\textcolor{blue}{Push-MOG makes the same assumptions as Agboh et al.~\cite{mogplane}: we assume the objects are extruded convex polygons, and have roughly uniform mass so that their centers of mass coincide with their geometric centroids.} %\textcolor{blue}{[FILL IN!!!]}

\subsection{State, Action, and Objective}

% We assumed the problem to be analogous to 2D grasping and pushing, we model the state and actions in 2D. However, motions may accidentally move or even knock over blocks. Thus, the scene is re-processed after every motion. Compared to the time needed to execute a step, however, this re-planning is negligible \textcolor{blue}{[TODO] if this is not true someone please correct me!}. However, similarly to \cite{mognet}, we will use certain concrete characteristics from the model -- in particular, when a set of objects provably cannot all be simultaneously grasped -- to guide the algorithm.
%and to avoid wasting time on grasps that cannot work.

Let the set of objects on the work surface be $O = \{o_0, o_1, \dots, o_{N_o - 1}\}$ where each $o_i$ is a convex object and $N_o$ is the number of objects on the work surface. % which we want to partition into a set of groups $G$. Each $g \in G$ (where $g \subseteq O$) should consist of objects which are close together and, when rearranged, can all be simultaneously grasped.
%
The robot executes a sequence of \emph{pushes} and \emph{transports}; each push translates and/or rotates a single object in the workspace without colliding with others, while each transport grasps aset of closely clustered objects and transfers them to the goal. %with the objective of clearing the work surface in the shortest amount of transport actions.

We divide this problem into three sub-problems:
\begin{enumerate}
    \item \emph{Clustering:} Divide the objects into clusters. No cluster should contain more objects than can be stably grasped by the gripper.
    \item \emph{Pushing:} Push the objects in each cluster close together.
    \item \emph{Transport:} Perform grasps (containing as many objects as possible each time) and transport the grasped objects to the goal until no clusters remain.%\footnote{The transport step does not make direct use of the cluster labels; rather, thanks to the pushing step, objects in a cluster should be close together and hence good candidates for MOG-Net computed multi-object grasps.}
\end{enumerate}
Due to the inherent uncertainty of working with real objects, a grasp might not get every object in a cluster, so a cluster may need multiple grasps to clear completely. The clustering step is also distinct in that it is purely computational and does not involve any physical action.

Since we don't optimize an explicit objective in the clustering or pushing problems, we instead use the characteristics of the problem to guide the choice of algorithm.
%Additionally, even given this broad algorithmic outline, there are multiple possible variations on how the algorithm is executed: for instance, two sensible ways to order the pushing and grasping steps are (i) execute all pushes first, then all grasps; (ii) iterate over all groups in some order, executing all the pushes on a group and then grasping and delivering it to the goal before moving onto the next group. There is also the question of whether re-clustering during the process is advantageous or not.

%In our implementation, we compute the groups once, then execute all pushes, and finally perform multi-object grasps until the workspace is clear.



%given a collection of extruded-object objects $O$ on a flat workspace, and robotic manipulator capable of pushing and grasping with parallel jaws, transport all the objects to a given goal area away from the workspace (typically a bin or box which can then be stored or shipped) in the shortest possible time. Since pushes can generally be executed faster than grasps and the objects are typically closer to each other than to the goal area, it is often more efficient to push objects closer together and transport them together to the goal than to transport them individually (the single-object grasp approach).



\subsection{The Clustering Problem} \label{sec:clustering-problem}

In the clustering stage, the goal is to partition the set of objects $O$ into clusters in such a way that (i) the objects in any cluster are close together and (ii) each cluster consists of objects that can be stably grasped together (provided they are pushed into an appropriate configuration). Finally, since the goal of clustering the objects is to reduce the number of grasps necessary to clear the workspace, a good overall clustering will partition the objects into as few clusters as possible, as each cluster roughly corresponds to one grasp. We denote the output of the clustering algorithm as a list of clusters $C$, and each individual cluster as $c \subseteq O$ (since a cluster is a set of objects).

In this problem, each object $o$'s position is represented by its geometric centroid, which we denote $M_o$. This allows the application of an appropriately modified version of the hierarchical clustering algorithm (which clusters points).

%A good `group' for multi-object grasping in general consists of several closely-clustered objects in a configuration which fits into the gripper width. The addition of the push action allows these conditions to be relaxed

An important characteristic of each object $o$ is its \emph{minimum final grasp diameter} $d^*_{o}$, corresponding to the minimum width of a stable single-object grasp on $o$. Then, given a cluster $c$, we denote the \emph{minimum grasp diameter of $c$} as $d^*_c = \sum_{o \in c} d^*_{o}$. The gripper also has a width $d^{\text{(gr)}}$, and if $d^*_c > d^{\text{(gr)}}$ we regard cluster $c$ as ungraspable (thus requiring division into smaller clusters)\footnote{It is possible that even if $d^*_c \leq d^{\text{(gr)}}$ the cluster does not have a stable grasp. For example, a cluster of three identical equilateral triangles cannot be stably grasped at all.}. %We do not formalize a concrete optimization problem for this; instead, we use the above as rough guidelines for selecting and designing a clustering algorithm, described in Section~\ref{sec:clustering}.

Also, it is important for the clusters to not interfere with each other during the pushing step, which might happen if clusters are spatially intermingled. While point clustering usually avoids this by default (such clusters are locally non-optimal), the grasp diameter constraint may make such a solution to be `optimal' unless it is specifically excluded. We thus add a constraint that for any $c_1, c_2 \in C$, the centroids of the objects in $c_1$ (i.e. the set $\{M_o : o \in c_1\}$) are linearly separable from the centroids of the objects in $c_2$.

%the convex hulls $\text{H}(\{M_o : o \in c_1\})$ and $\text{H}(\{c : o_i \in g_2\})$ are disjoint (or, equivalently, that there is a line separating the sets $\{c_i : o_i \in g_1\}$ and $\{c_i : o_i \in g_2\}$).


The clustering problem is then defined to partition $O$ into a set of clusters $C$ such that: (1) $d^*_c \leq d^{\text{gr}}$ for all $c \in C$; (2) any $c_1, c_2 \in C$ have a line which separates the centers of mass of the objects they contain; (3) each cluster has small pairwise distances between its objects; and (4) there are few clusters overall. It is solved using a modified hierarchical clustering algorithm. \footnote{Since we don't optimize over an explicit objective function we do not define one.}

\subsection{The Pushing and Grasping Problems}

After the clusters have been defined, the next step is to push each cluster closer together to make multi-object grasping more effective (see Fig.~\ref{fig:push_alg} for an illustration). We assume that (due to the separating line constraint in the clustering problem) each cluster can be treated as a separate instance of the pushing problem.

%\subsection{The Grasping Problem}

Finally, once the pushing is done, we move the objects to the goal via multi-object grasping. As in \cite{mognet}, the objective is to move the objects to the goal with as few grasps as possible (without pushing, as that has already been done).

\begin{figure}[t]
    \vspace{0.2cm}
    \centering
    {\includegraphics[width = \linewidth]{images/pushing_alg.png}}
    % {\includesvg[width=85.5mm]{images/ObjectGroupingMOG.svg}}
    \caption{{Example of push-planning for polygonal clustering. Objects outlined in solid black lines are objects being pushed towards the object with the closest face to them. The objects outlined in dashed lines are the objects' respective final locations after being pushed. The cluster now has objects that fit within the gripper's width and can proceed to grasp them. }}
    % \vspace{-0.7cm}
\label{fig:push_alg}
\end{figure}

%In order to effectively use multi-object grasping, we need a way to determine which objects to grasp together, which suggests a clustering approach. In general, such groups should be: (i) positioned relatively close to each other, and (ii) not too large to grasp simultaneously. While randomly scattered objects may be unlikely to fall into convenient closely-grouped clusters, the addition of a pushing action allows 
%condition (i) to be somewhat relaxed since the robot can now push objects in a cluster together before grasping (though it is still not efficient to group objects which are scattered too far apart); the benefit of doing so is that pushes are generally faster to execute than grasps, so it is worth it to use pushes to reduce the number of grasps needed. 
%condition (ii) to be relaxed: since the blocks will be pushed together before being grasped, whether a group is `graspable' is not determined by their current positions and orientations but by their sizes and shapes.

%\subsection{Assumptions}

%As in [CITE], we consider only antipodal grasps and assume that all objects are extruded convex objects with friction coefficient $> \mu$ for some $\mu \geq 0$, which is known to MOG-Net.

%\subsection{The grasp diameter constraint}



%\subsection{Goal and problem}

%Since the goal is to identify groups of objects which can then be quickly and conveniently pushed into configurations which will allow for efficient multi-object grasping, the full problem contains a great deal of complexity and uncertainty. Thus, we use the hard diameter constraint and the general rule that closely-grouped objects will be faster to push into a graspable position as guidelines for our clustering algorithm (Section~\ref{sec:usup_clust}).




==> old_versions/section-4-clustering.tex <==
\section{\algo{} Algorithm}
The \algo~Alg. (\ref{alg:algo-overview}): After perceiving an initial scene, we find a cluster of objects which are not only close to each other but also can fit inside the gripper. From there, we plan and execute a series of push actions to bring together the clustered objects so they are touching each other. Now, we query MOG-Net algorithm \cite{mognet} to clear that cluster through Multi-Object grasps. Below, we outline how the \algo~algorithm plans and executes these steps.



\setlength{\textfloatsep}{2mm}
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Parameters}{Parameters}
    \SetKwInOut{Subroutines}{Subroutines}
    \Input{$I$: Image of the workspace}

    Capture and parse workspace image $I$ into a 2D object map of all objects $O$\\
    Partition $O$ are into clusters $C$ (Alg. 2, see \ref{sec:clustering})\\
    \For{cluster $c \in C$}{
        Plan the pushes, $P$ (Alg. 3, see \ref{sec:push})\\
            \For{push $p \in P$}{
                Calculate post-push location of the pushed object
            }
        Update the state of the simulated workspace\\
        Run MOG-Net (\ref{sec:MOGnet}) to identify grasp MOG $g$ for cluster $c$ \\
        Execute $g$ to remove $c$\\
    }
    % Run MOG-Net (\ref{sec:MOGnet}) to identify the grasps $p$ in the workspace \\
    % \If{$len(p) == len(O) \& len(O) != 1$}
    % {Go to step 1 and repeat planning}
    % \Else{
    %     Execute the planned grasp and remove \\
    % }
    \caption{\algo{}}\label{alg:algo-overview}
\end{algorithm}
\setlength{\floatsep}{2mm}

\subsection{Clustering Details}\label{sec:clustering}

As described in Section \ref{sec:clustering-problem}, the goal of this step is to cluster objects into graspable clusters. In order to accomplish this we compute the centroids of each object and use a bottom-up hierarchical clustering. We find the largest bounding box that encloses each object and cluster them into clusters based on their proximity to each other. Once these clusters are formed, we check that the sum of the widths of all the objects in the cluster does not exceed the width of the gripper. If we encounter a non-valid cluster $c$ (i.e. such that $d^*_c > d^{\text{gr}}$), then we split $c$ into two clusters $c_1, c_2$ using a separating line (objects are divided based on their centroids), minimizing the difference in cluster diameter $|d^*_{c_1} - d^*_{c_2}|$. %\textcolor{red}{The initial division is done by drawing a line diagonally and rotating it by 45$^\circ$ on both sides. To find the most optimal division boundary, we minimize the difference of the sum of the widths between the two clusters. We make sure to repeat this process until all clusters are valid and fit the gripper constraints.}

%See Fig.~\ref{fig:polygroup} for an example of push planning output.



\setlength{\textfloatsep}{2mm}
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Parameters}{Parameters}
    \SetKwInOut{Subroutines}{Subroutines}
    \Input{$O$: List of objects}
    \Output{$C$: List of clusters}

    Compute centroids $M_{o}$ for all $o \in O$ \\
    Hierarchical clustering on $\{M_{o} : o \in O \}$ to generate clusters $C$\\
    Check the validity of each cluster $c \in C$ based on max gripper width\\
    \For{non-valid cluster $c \in C$}{\textcolor{red}{
        Minimize weight $W$ on $\theta$ using the following:
        \For{$\theta \in [-{\frac \pi 4}, {\frac \pi 4}]$}{
            $v = \langle\cos\theta,\sin\theta\rangle$\\
            Split the objects into two clusters $c_{1}, c_2$ across this line \\
            Calculate weight difference $W = |\sum_{o\in c_1} d^*_o - \sum_{o\in c_2} d^*_o|$}
            %, where $w$ is the minimum grasp width of the object
        }
        Split the cluster on this $\theta$
    }
    %All object clusters are valid and fit within the gripper constraint\\
    \caption{Clustering Algorithm}\label{alg:algo-overview}
\end{algorithm}
\setlength{\floatsep}{2mm}

%Minimize weight $W$ on $\theta$ using the following:
        %\For{$\theta \in [-{\frac \pi 4}, {\frac \pi 4}]$}{
            %$v = \langle\cos\theta,\sin\theta\rangle$\\
            %Split the objects into two clusters $c_{1}, c_2$ across this line \\
            %Calculate weight difference $W = |\sum_{o\in c_1} d^*_o - \sum_{o\in c_2} d^*_o|$


\subsection{Push Planning}\label{sec:push}

%Common problems that arose when pushing objects were that they would topple over when pushing them from one location to the next. 

\textcolor{blue}{Push planning considers how to push objects in a cluster closer together in order to facilitate the final grasping stage. This can be broken into two steps: (i) determining the desired locations of the cluster's objects; (ii) computing the parameters of the pushes to get them there. For object $o$, we denote the desired location of its centroid as $M'_o$, which is chosen both to make pushing easier and to position the objects for grasping. For simplicity, we only specify a desired location for the centroid (and not a desired orientation). All pushes are executed in one motion in a straight line; the direction and distance that $o$ is pushed is given by the vector $M'_o - M_o$ (to move its center of mass from $M_o$ to $M'_o$).}

\textcolor{blue}{For executing a push with a parallel-jaw gripper, we propose the technique of \emph{fork pushing}: we angle the gripper so the line between the jaws is perpendicular to the desired push direction. This allows the gripper to push both along an edge or around a vertex of an object (see Fig.~\ref{fig:polypush}), whereas a flat-edged pusher could not push against a vertex without the object undergoing a major rotation.}

%\textcolor{blue}{Once a desired location is determined for an object, Push-MOG determines (a) what width to set the gripper jaws to; (b) what angle to set them at; (c) where on the object's edge to set the gripper. The direction of the push is determined by the difference between the desired location and the current location of the object's centroid.}

%Push-MOG plans pushes based on whether the desired direction of motion can be achieved by pushing on a single side of the object or whether i. 
%If in order to push an object from its initial position to its final position, it is in a configuration where the flat surface is perpendicular to the pushing vector then we open our gripper to cover 75\% of the edge's surface area. This is also true for objects where the two joining edges form an angle greater than or equal to 90$^\circ$. However when we are pushing objects whose vertex is along the vector of motion then it is preferable to open the gripper (x amount \textcolor{blue}{[Eh??]}) so that the corner of the object fits nicely into the gripper.


%See Fig.~\ref{fig:polypush} for an example of push planning output.

\setlength{\textfloatsep}{2mm}
\begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Parameters}{Parameters}
    \SetKwInOut{Subroutines}{Subroutines}
    \Input{$C$: List of Clusters}
    %\Parameters{$COM$: Center-of-mass algorithm of choice}
    \Output{$v_{start}, v_{end}$: Start and end push points for each object}

    \For{valid cluster $c \in C$}{
        $M_c = \frac {\sum_{\text{object } o\in c} M_o}{|c|}$\\
        $m = \argmin_{o\in c} \|M_o - M_c\|$, the central object in the cluster\\
        \For{object $o \in c \backslash m$}{
            $v = M_o - M_m$\\
            Calculate center of furthest edge $e_o$ of object $o$ to $m$ on $v$\\
            Calculate closest edge $e_m$ of object $m$ to $o$ on $v$\\
            Scale and translate $v$ to capture the length of the push vector\\
        }
    }
    \caption{Push Planning Algorithm}\label{alg:algo-overview}
\end{algorithm}
\setlength{\floatsep}{2mm}

\subsection{MOG-Net Integration}\label{sec:MOGnet}
Following the pushing step, we use MOG-Net \cite{mognet} on the clusters to clear the workspace. 
%
%As described in  (Agboh et al.), the algorithm clears the workspace, by optimizing the number of picks and places required. First, the system will identify a cluster that can be cleared from the workspace, and then generate grasps which will achieve this goal. The initial approach to this was splitting the MOG-Net and \algo~work, so that the objects would be pushed into their clusters and then cleared. 
%
To improve efficiency, we use the simulated coordinates of the push action to plan grasps instead of taking an image of the workspace again.

However, this process is not fully robust, because pushes may cause other blocks in the way to deviate from their estimated location, leading to a faulty grasp. 

To remedy this, whenever a transport is performed (thus moving the gripper out of the camera's view of the workspace), a new image of the workspace is taken, allowing these errors to be corrected; the algorithm also uses this image to re-plan the clustering (\ref{sec:clustering}) and pushing (\ref{sec:push}) on the remaining blocks (which may have been pushed aside or missed during an earlier grasp).

\input{figures/example_groups}
\input{figures/example_push}



==> old_versions/section-5-experiments.tex <==
\section{Experiments and Results}\label{sec:experiments}

To evaluate the performance of the policies developed in the paper, we run experiments in a real workspace. %These experiments aim to quantitatively measure the performance of \algo~and investigate the strengths and weaknesses of our methodology. %Thus, this section will overview our setup, experiments, and results.

\subsection{Experimental Setup}\label{sec:expsetup}

An example input is shown in Fig.~\ref{fig:wksp_scatter}. We use a Universal Robotics (UR) 5 Robot with a Robotiq 2F-85 gripper mounted to its wrist. We perform experiments on 34 convex objects which range from 3-sided to 8-sided; \textcolor{blue}{we excluded some of the objects from the original MOG-Net experiments \cite{mognet} which were too thin and hence tended to topple when pushed. We note that this implies that Push-MOG should only be used with objects that are sufficiently stable.} All experiments assume a random placement of the objects in the workspace, and 4 of 5 such configurations are shown in Fig.~\ref{fig:wksp_scatter}. To generate a random placement, we uniformly sample the workspace and create circles that encompass the max radius of any object we are using. Before creating each circle we ensure that they do not overlap, and continue sampling the object set without replacement until all objects are placed. Then a human sets up the configuration in real, mirroring the randomly generated image. We generated 5 random scenes, on which we will perform all experiments. 
%
%All of these objects are frictional on their graspable edge faces, which are on the same 2D plane as the grippers at all times. 
%
We add friction on the graspable faces of the objects by wrapping them in frictional tape. 

To perceive the environment, we use an Intel RealSense L515 Camera, which outputs RGB-D images, mounted directly above the workspace. 
%
%This camera is mounted above the robot workspace, with a field of view parallel to it, and used to capture images of the workspace. 
%
To calibrate the Camera-Robot transform, use an ArUco marker \cite{aruco} which is manually calibrated with an accuracy of \textcolor{blue}{$\sim 2mm$}. %The object vertices, $O$, extracted lie in the robot plane, measured in meters from the robot's home position of $(0,0,0)$ in the XYZ space.

The pushing action consists of 5 repeated steps:
\begin{enumerate}
    \item Open the jaws to 25 percent width
    \item Move the gripper above the desired push location
    \item Move down to the object's Z-height
    \item Move the gripper and push it to its planned location
    \item Move the gripper above its planned location
\end{enumerate}

The Multi-Object Grasping action is an executed with the MOG-Net algorithm \cite{mognet}. Here we repeat the following:
\begin{enumerate}
    \item Plan a grasp for each cluster
    \item Move the gripper above the desired grasp location
    \item Open the jaws fully
    \item Move down to the work surface
    \item Close the jaws to complete the grasp
    \item Move the gripper outside the workspace and open the jaws fully to drop the objects
\end{enumerate}

\subsection{Baselines}

\textcolor{blue}{We compare Push-MOG against two baselines: Frictional SOG, which uses single-object grasps, and MOG-Net \cite{mognet}, which uses multi-object grasps but does not use additional actions to help group the objects together.}

\begin{enumerate}
    \item \textbf{Frictional SOG}: This is the same as one of the baseline algorithms proposed in the MOG-Net paper \cite{mognet}, which randomly chooses one object at a time to remove from the workspace and executes its optimal grasp. \textcolor{red}{However, we introduce one minor change to this baseline. Initially, SOG would remove objects in the order of green, yellow, red, and then blue. However, this choice adds nothing to the algorithm, so we randomize which object will be cleared next.}
    \item \textbf{MOG-Net}: This baseline follows the main technique in the MOG-Net \cite{mognet}~paper, which is run without pushing.
\end{enumerate}

% \subsection{\algo}\label{sec:pushmog_algo}

\subsection{Results}\label{sec:results}


\textcolor{blue}{Our main results are given in Table~\ref{tab:results}. We find that randomly-placed objects are not generally positioned well for multi-object grasps (as TPO is almost exactly the same between MOG-Net and Frictonal SOG, which does not attempt mutli-object grasps), thus requiring the use of auxiliary actions such as pushes to facilitate multi-object grasping. Indeed, the performance of Frictional SOG and MOG-Net are almost identical, suggesting that there are few, if any, `naturally occurring' multi-object grasps in a typical scene of randomly-scattered objects. \algo~successfully uses the pushing actions to generate graspable object clusters, which reduces TPO by roughly $25\%$. This comparatively modest reduction in TPO (as compared to the experimental results on the original MOG-Net \cite{mognet}) is due to two factors: the objects are randomly placed and hence not naturally amenable to being grasped more than two at a time; and the use of only stable objects, which tend to have larger diameters which limits the number that can be grasped simultaneously.}

\textcolor{blue}{However, we note that Push-MOG yields a lower PPH in our experiments than the baseline methods. This is due to the time taken to execute push actions and the fact that our experimental setup (with a stationary arm) is limited to having the bin close to the work surface; since the value of reducing the number of transports increases proportionally to bin distance, this means that our experimental setup does not yield high reward for reducing the number transports. Nevertheless, by using both TPO and PPH measured in our experiments, we can study the relative performance of Push-MOG and Frictional SOG under different bin distances by adding in the extra time per transport. Specifically, we ask: how long would a transport need to take for Push-MOG's reduction in transports to be worth the extra time spent on pushes? Push-MOG loses $\frac{3600}{250.16} - \frac{3600}{331.70} = 3.54$ seconds per pick compared to Frictional SOG; however, it saves $1.01 - 0.75 = 0.26$ transports per pick. Thus, if each transport takes an additional $\frac{3.54}{0.26} = 13.62$ seconds, then Push-MOG will have a faster overall pick rate (estimated PPH with additional transport time) than Frictional SOG. We estimate the average transport time in our setup from Frictional SOG; it is approximately $\frac{3600}{331.7 \cdot 1.01} = 10.75$ seconds per transport ($331.7$ picks per hour times $1.01$ transports per pick means approximately $331.7 \cdot 1.01 = 335.02$ transports per hour). Hence, estimated PPH is approximately equal if transport time is increased to $13.62 + 10.75 = 24.37$ seconds.}

%We find that \algo~efficiently generates multi-object grasps after pushing, and it compares fairly with multi-object grasping without pushing.

%\algo{}'s significantly lower TPO stems from its generation of efficient pushes. These pushes allow for robust Multi-Object grasps which are key in reducing the number of trips the robot needs to make to the bin when clearing the workspace.

%Although the TPO is better, the time it takes for the system to clear the workspace is higher, leading to a lower PPH. One reason for the slower performance of \algo~is the time it takes to push. The algorithm generates multi-object grasps but its full potential could be realized when the box is farther away from the table. In this way, multi-object grasps will play a more significant role as it reduces the total number of trips to the box, along with further improvements to push planning and execution speed.


\input{figures/results_general}
\input{figures/wksp_scattered}
